Target-Guided Dialogue Response Generation Using Commonsense and Data Augmentation

Target-guided response generation enables dialogue systems to smoothly transition a conversation from a dialogue context toward a target sentence. Such control is useful for designing dialogue systems that direct a conversation toward specific goals, such as creating non-obtrusive recommendations or introducing new topics in the conversation. In this paper, we introduce a new technique for target-guided response generation, which first finds a bridging path of commonsense knowledge concepts between the source and the target, and then uses the identified bridging path to generate transition responses. Additionally, we propose techniques to re-purpose existing dialogue datasets for target-guided generation. Experiments reveal that the proposed techniques outperform various baselines on this task. Finally, we observe that the existing automated metrics for this task correlate poorly with human judgement ratings. We propose a novel evaluation metric that we demonstrate is more reliable for target-guided response evaluation. Our work generally enables dialogue system designers to exercise more control over the conversations that their systems produce.

==> method_old.tex <==
% \section{Task Background}
\section{Task Overview}
\label{sec:background}
We first formalize the task of target-guided response generation. 
Given a conversation history of n utterances $C= \{u_1,u_2,...,u_{n-1}\}$ between two speakers A and B, and a target $t$ for speaker B's turn $u_n$, the task is to generate a transition sentence $s$ which serves as a smooth link between the context and the target. The target can be defined in terms of a phrase or a sentence. \textit{Otters} dataset~\cite{DBLP:conf/acl/SevegnaniHKR20} consists of a simplified setting of one-turn topic transitions, where the conversation history consists of a single utterance $u_a$, and a target utterance $u_b$ and the task is to generate a transition utterance $s$ to serve as a smooth link between $u_a$ and $u_b$. 
The task is challenging since a system needs to devise a strategy that balances the competitive objectives of generating a response which is coherent to the context, while smoothly driving the conversation towards the target.
% The aim is to achieve smooth transitions by generating a response natural to the conversational context, and drive the conversation towards the target.
% A system agent needs to apply a good conversation strategy to make a trade-off between these two competitive objectives. 




% \section{Methodology Overview}
% \label{sec:methodology}

In this work, we propose two approaches for the transition response generation task: 1) Commonsense-guided response generation (\autoref{sec:commonsense}), and 2) Data augmentation to tackle data sparsity (\autoref{sec:augmentation}).
We refer to the proposed method as \textbf{\coda{} (Commonsense Path and Data Augmentation)}.
We also propose a novel metric \textbf{\metricname{}} to automatically evaluate the smoothness of response transitions (\autoref{sec:tcmetric}).



\begin{figure*}[tb]
    \centering
    \vspace{-.2pc}
    \includegraphics[width=0.96\textwidth]{images/model-overview-naacl6.jpg
    % images/model-overview.pptx2.jpg
    }
    \vspace{-.5pc}
    % \caption{ \small Overview of Commonsense Response Generator (CRG) model:
    % During training, the Knowledge Path Generator model KPG-wc is fed the entities from the context, target and the gold transition response, and the output path from KPG-wc is used in CRG model's training. During inference, KPG-ht model is fed the context and target entities and the model generates a path with new entities such as ``vacation''. CRG model conditions on this path for transition response generation.   }
        \caption{ \small Model illustrations for KPGs - Knowledge Path Generators (left) and CRG - Commonsense Response Generator (Right). Base architecture for all models is GPT-2. Given a path sampled from ConceptNet, KPG-wc learns to predict the path given the head, tail and intermediate entities of the path while KPG-ht learns to predict the path given only the head and tail entities.  
        For the CRG model, during training, a head entity from the context, a tail entity from the target and intermediate entities from the gold transition response are fed into KPG-wc and its output path is used as input to the CRG model. During inference, a head entity from the context and a tail entity from the target are fed into the KPG-ht model. KPG-ht then generates a path with new concepts such as ``go on vacation''. CRG model conditions on this path for transition response generation.   }
    \label{fig:interface1}
    %  \vspace{-1em}
\end{figure*}

\section{Commonsense-Guided Response Generation}
\label{sec:commonsense}
% -- Need for commonsense 
We frame the target-guided response generation task as follows. %a typical dialogue response generation problem where 
Given a conversation history of n utterances $C= \{u_1,u_2,...,u_{n-1}\}$ and a target $t$, a conditional language model learns to predict the tokens of the transition response $s$ by minimizing the cross entropy loss of the ground truth transition response.

As mentioned previously, target-guided generation can potentially benefit by incorporating commonsense reasoning. 
Pre-trained models %have been demonstrated to show good performance on typical response generation tasks and encode certain commonsense reasoning abilities~\cite{trinh2018simple}. However, %our task is challenging due to a lack of abundant training data, and requires complex commonsense reasoning to generate smooth transitions by relating concepts between the context and the target. 
% such models 
are 
%also 
known to suffer in cases where commonsense knowledge is required during generation~\cite{ijcai2018-643, Guan_Wang_Huang_2019}, especially in tasks where there is not enough data available for learning commonsense patterns from the text, which is true for our case.
In contrast, Commonsense Knowledge Graphs 
%(CKGs) 
like ConceptNet~\cite{speersConceptnet} provide structured
knowledge about entities, which enables higher-level reasoning about concepts. 
%
% -- Explain what we do
In this work we use commonsense knowledge from ConceptNet for planning a %and reasoning to generate the 
transition response. ConceptNet is a large-scale semantic graph that has general phrases as nodes and the commonsense relationships between them, such as `IsA' and `AtLocation'
% and `Synonym'.
%Using knowledge from the ConceptNet knowledge graph (KG), however, poses a major challenge. %the following challenges: 1) 
However, ConceptNet consist of non-canonicalized text and hence suffers from severe sparsity~\cite{malaviya2020commonsense}. Therefore, it is not always possible to find the concepts and connections between context and target concepts. %2) We need to select and align relevant knowledge from the KG. However, unavailability of such ground truth annotations, high cost of human annotations, and heterogeneity of ConceptNet makes it difficult. %Using incorrect knowledge can hurt the model's reasoning capabilities.   

To address the sparsity issue, we develop Knowledge Path Generator (\textbf{KPG}), a language model that generates knowledge instead of retrieving it from KG. The model takes a pair of entities or concepts as input %from the context and the target,
and generates a multi-hop path connecting the two. Since the knowledge is generated, the path may not exist in ConceptNet and may contain nodes not actually present in KG. Thus the generated knowledge generalizes over the facts stored in the KG (Section~\ref{sec:pathgenerator}). %We train a GPT-2~\cite{radford2019language} based model on the paths sampled from ConceptNet, described in more detail in section~\ref{sec:pathgenerator}. 
% After sampling multiple paths between two entities, From the paths sampled our approach described in section XXX selects the most relevant paths aligned with the ground truth response. 

To generate commonsense based responses, we train a Commonsense Response Generator (\textbf{CRG}) model to generate the transition response conditioned on the paths generated by the KPG model (Figure \ref{fig:interface1}). Conditioning the response generation on commonsense paths improves the reasoning capabilities of the CRG model and provides the added benefits of interpretability and control over the generation process.
% represents the overview of our proposed approach. 
 
%why generative commonsense
%interpretability/controlability, sparsity, generalizability



\subsection{Commonsense path generator}
\label{sec:pathgenerator}
%The objective of t
The KPG model attempts to connect an entity phrase or topic from the context with an entity from the target by creating knowledge paths between them.

\noindent
\textbf{Path Sampling:} 
% \textbf{Training Data} 
To create training data for the KPG model, we sample paths between entity phrases from ConceptNet using random walks. This step builds upon past work of \citet{wang-etal-2020-connecting}.
Given the ConceptNet graph with a set of nodes $N$ and edges $E$, we perform random walks on the graph to sample a set of paths $P$ of the form $p=\{n_0,e_0,n_1,e_1,...,e_{k-1},n_k\}\in P$. Here, a path $p$ connects a head entity phrase $n_0$ with the tail entity phrase $n_k$ via intermediate entities and edges (or relations) $n_i, e_i$. 
To sample paths, the random walk begins with a random entity node $n_0$ and samples a path of random length $k \in \{1,2,...,K\}$, where we have set $K=6$ in this work.
To sample paths that are useful for our task, we prevent sampling certain edges types such as \textit{Synonym} (Appendix~\ref{sec:edges}). %Since the nodes in ConceptNet are directional, we also add inverse edges during path sampling.  

\noindent
% \textbf{Training the KPG model:}
\textbf{KPG-head-tails (KPG-ht):}
The paths sampled from the KPG model are fed to the CRG model to provide it with relevant commonsense knowledge.
%used by the CRG model as conditioning to improve its commonsense properties. Therefore, its important to only generate paths which are relevant, and align with the context and target concepts during inference, and additionally to the transition response during training.
When using CRG at inference time, we use a language model (referred to as \textit{KPG-ht}) to construct commonsense paths linking a head and a tail entity.
For the \textit{KPG-ht} model, the input is just the head entity $n_h$ and the tail entity $n_t$. 
For a sample path $p=\{n_h,e_0,n_1,e_1,...,e_{k-1},n_t\}$, 
the path is formatted into the following sequence ``[target] $n_t$ [sep] $n_h$ $e_0$ $n_1$ $e_1,…,e_{k-1}$ $n_t$''. Thus the model is trained to output a path sequence given the head entity $n_h$ and the tail entity $n_t$ as input.
%Note that 
KPG-ht is used only during inference phase of the CRG model. %, described in the next section. 


\noindent \textbf{KPG-with-contains (KPG-wc):}
We note that there can be a large number of possible paths for a given entity pair. Moreover, we do not have ground truth annotations regarding which path is relevant for a given response. Irrelevant commonsense paths might discourage the CRG model to condition on the provided commonsense knowledge. Thus, to train CRG model, we would prefer paths which are somewhat aligned with the ground truth response. We achieve this by considering a separate model KPG-with-contains (KPG-wc) to be used during training phase of CRG model. %In addition to head and tail entity, \textit{KPG-wc} also admits a set of keywords to be contained in the output path. %version of the KPG model. %Next we will describe  KPG-wc model. % for preparing training data.
% Therefore, we create two versions of the KPG model using the sampled paths, the model \textbf{KPG-with-contains (KPG-wc)} for preparing training data and model \textbf{KPG-head-tails (KPG-ht)} for preparing test data for the CRG model.


% For the 
\textit{KPG-wc} %model, we train 
is a conditional generation model where the input comprises of a head entity phrase $n_h$, a tail entity phrase $n_t$ and a pre-specified entity set $E_p$ which should be contained in the generated path. 
% The path is formatted into a sequence of natural language tokens. 
% In figure XXX, given a head entity $n_h$, the tail entity $n_t$ and a sample path $p=\{n_0,e_0,n_1,e_1,...,e_{k-1},n_k\}$, 
For a sample path $p=\{n_h,e_0,n_1,e_1,...,e_{k-1},n_t\}$, 
the path is formatted into the sequence ``[wc] k1 [wc] k2…[target] $n_t$ [sep] $n_h$ $e_0$ $n_1$ $e_1,…,e_{k-1}$ $n_t$''. Here ``wc'' symbolizes ``will contain''. The set $E_p = \{k_1, k_2,...,k_n\}$ used in the sequence is a randomly permuted sequence of entities  $n_1, n_2,…, n_{k-1}$ of the sampled path. 
Training with this sequence indicates to the model that the path generated between $n_h$ and $n_t$ should contain the entities from the set $E_p$ in a sensible order. Specifying the special token ``[target]'' followed by the tail entity $n_t$ informs the model about the last entity it should output when generating a path. We discuss how the set $E_p$ is constructed for training the CRG model in the next section.

% For the \textit{KPG-ht} model, the input is just the head entity $n_h$ and the tail entity $n_t$. 
% For a sample path $p=\{n_h,e_0,n_1,e_1,...,e_{k-1},n_t\}$, 
% the path is formatted into the sequence ``[target] $n_t$ [sep] $n_h$ $e_0$ $n_1$ $e_1,…,e_{k-1}$ $n_t$''. Thus the model is trained to output a path sequence given the head entity $n_h$ and the tail entity $n_t$ as input.
% This model is used only during inference of the CRG model, described in the next section. 


\subsection{Response generator}
\label{sec:responsegenerator}
The Commonsense response generator samples and aligns the paths generated using the KPG model and uses it for generating commonsense knowledge conditioned transition responses. %We show the overview of this model in Figure \ref{fig:interface1}.

\vspace{1mm}
\noindent
\textbf{Entity extraction}.
We extract a set of entities $E_h, E_t$ and $E_r$ from the context, target and gold transition response respectively. We first run NLTK's part-of-speech tagger on a sentence, and then use NLTK's chunker to extract the set of noun and verb phrases present in the sentence. % (more details in Appendix XXX). 
Additionally, we design simple grammar rules (details in Appendix) to convert some phrases to more concise forms (for example, ``watching the star'' is converted to ``watch stars''). This step is done to make the entities more similar to the kind of nodes present in ConceptNet. 

\vspace{1mm}
\noindent
\textbf{Sampling and filtering paths:}
% \textbf{Path Filtering:}
In this step, for every pair of head and tail entity from $E_h$ and $E_t$, we sample multiple paths from the KGP models using topk sampling and chose one or more of these paths for training and inference. 
\textit{For training} the CRG models with the commonsense paths, we need to curate paths that are relevant to and aligned with the gold response so that they are not ignored by the CRG model during inference. We achieve this by first sampling paths which are relevant to the ground truth response, and then apply filtering mechanisms to curate the final set of paths. For training data path sampling, we use the \textit{KPG-wc} model. The input to the model is a head and tail entity pair $n_h$ and $n_t$, and the entity set $E_p$ that consists of the set of entities $E_r$ from the gold transition response. The model then generates a set of paths that contain the head and tail entities as well as the gold response keywords. Thus, the sampled path is inherently relevant to the gold response due to the conditioning on gold keyword entities. During inference, the set $E_r$ is not available, so we leverage the  \textit{KPG-ht} model that takes just the head and tail entity pair $n_h$ and $n_t$ as input to generate a commonsense path.

Assuming the context and target consists of $m$ and $n$ entities each, and we sample $q$ number of paths per pair, we get a total of $m\times n \times q$ number of paths for each data instance.
%talk about keyword filtering
Since $m\times n \times q$ can be a large number, we use simple methods to sub-select entity pairs and paths. 
\textbf{(1)} Sub-selecting Entity Pairs: We score an entity pair %the set of $m\times n$ entities
by calculating the inverse document frequencies (computed using Gutenberg English corpus) of the entity tokens and summing up the maximum value found for a token in each entity in the pair. For training phase, we keep the top $D$ pairs of entities, and for testing phase we keep only the highest-scoring pair.
\textbf{(2)} Sub-selecting paths: We apply the following strategies to prune the set of paths for each entity pair: 1) \textit{Perplexity} - We filter out all the paths whose perplexity values (from the KGP models) are more than double the average perplexity values of all paths between an entity pair. 2) We remove all the paths which have repetition of entities since repetition often leads to degeneration during decoding. 3) For paths in training data, we filter out paths which contain entities not present in the gold response. After filtering out such paths, we have a final set of $P$ paths per response.
The paths from set $P$ are converted into natural language by converting the relation and inverse relations into textual format. For example, ``art gallery UsedFor for art'' is converted to ``art gallery is used for art''.

\vspace{1mm}
\noindent
\textbf{Training and inference in CRG model}. The CRG model is trained as a conditional model with the following input sequence: ``\textit{knowledge path} [target] \textit{target sentence} [context] \textit{context sentence} [response] \textit{transition response}'' for each \textit{knowledge path} from the set $P$. We train the CRG model by minimizing the log-likelihood loss of the transition response $r$ given the context C, target T, and the path $p$.
%$$\mathcal{L}_{\text {r}}=-\sum_{i=1}^{l} \log P_{\theta}\left(r_{i} \mid r_{<i}, c, t, p\right)$$
For inference, we first create the set of paths $P$ by entity extraction, path  sampling and filtering and choose a random path $p$ from the final set $P$. The model then generates the transition response conditioned on the sequence of $c, t$, and $p$.






\section{Data Augmentation}
\label{sec:augmentation}
The task of target-guided response generation is still a relatively unexplored task, and Otters~\cite{DBLP:conf/acl/SevegnaniHKR20} is the only suitable dataset for this task to the best of our knowledge. 
% However, Otters is small and consists of only a few hundred context-target pairs with a few transition responses for each pair. 
However, Otters is small and consists of only a few hundred context-target pairs.
This makes learning transition concepts and strategies challenging in this low-resource setup. On the other hand, there are many publicly available dialogue datasets for training response generation models.
Such datasets contain free-flow conversations, where although the speakers generate context coherent responses, they do not condition their responses on any target. We propose a technique to leverage and re-purpose such datasets for the task of target-guided response generation. We pick the Dailydialog~\cite{li-etal-2017-dailydialog} dataset for experimentation and convert its conversations to target-guided conversations in two steps: 1) Target creation, and 2) Data filtering. 



% \begin{figure}[h]
%     \centering
%     \vspace{-.2pc}
%     \includegraphics[width=0.45\textwidth]{images/augmentation.png}
%     \vspace{-.5pc}
%     \caption{
%     \small An example to demonstrate how a conversation in DailyDialog can be re-purposed for the task of target-guided response generation. %We break a response into sentence clauses, and pick one of the clauses as target. 
%     }
%     \label{fig:aug}
%     \vspace{-.2pc}
% \end{figure}



\begin{table}[h]
\centering
\small
\begin{tabular}{lp{0.32\textwidth}}
\toprule
Context       & the restaurant looks authentic european.                   \\
Response      & the chef trained in florence. the pasta tastes nice here.  \\
SRL Output    & predicate = tastes, arguments= the pasta; nice here        \\
Target clause & the pasta tastes nice here. \\
\bottomrule
\end{tabular}
 \captionof{figure}{
    \small An example to demonstrate how a conversation in DailyDialog can be re-purposed for the task of target-guided response generation. %We break a response into sentence clauses, and pick one of the clauses as target. 
    }
    \label{fig:aug}
    \vspace{-.2pc}
\end{table}

For \textit{target creation}, we run Semantic Role Labelling (SRL) to predict predicate and arguments in a response. For each predicate identified, we create a clause by putting together the predicate and arguments in a textual sequence. Finally, we only use the clause occurring towards the end of the response as a target. 
An example for target creation is shown in Figure \ref{fig:aug} (Details about clause identification in Appendix~\ref{sec:clause}).
% An example target creation is shown in \autoref{fig:aug}, showing how we break a response into sentence clauses, and pick one of the clauses as the target. (Details about clause identification in Appendix~\ref{sec:clause})
%. For example, given a context ``Is my booking complete?'' and the response  ``your reservation is confirmed. now i need your phone number,'', we extract a clause $t$ ``i need your phone number'' as the target candidate $t$. 
% For clause extraction we use Allennlp's SRL parser~\footnote{github.com/allenai/allennlp} which is trained using a BERT-based model~\cite{shi2019simple} and is based on PropBank~\cite{palmer-etal-2005-proposition}. It identifies the arguments associated with the predicates or verbs of a sentence predicates (verbs or events) in a sentence and classifies them into roles such as agent, patient and instrument. %For the example above, it identifies ``need'' as a predicate with agent ``i'' and instrument ``your number''. 


% In \textit{data filtering} step, we filter out instances which are not suitable for target-guided generation. 
The target creation step does not guarantee that a candidate response transitions smoothly towards the target clause. 
% In the example above, the transition response "your reservation is confirmed." is coherent to the context, but does not transition well towards the target. 
% We filter out such instances by using a metric to score the coherence of transition responses towards the context and target. 
In \textit{data filtering} step, we use a \metricname metric to score a transition response in terms of its coherence to the context and the smoothness towards the target. The metric is described in more detail in section~\ref{sec:tcmetric}. The metric assigns a score between 0-1 for a transition response and we remove instances with a score less than a threshold $k$ (set to 0.7) from consideration. The remaining instances are used for pretraining response generation models which are finally fine-tuned on the Otters dataset.



\section{Target-Coherence Metric} 
\label{sec:tcmetric}
Evaluating target-guided responses is a challenging task as a good transition response needs to be both - coherent to the context and smoothly transition towards the target. Furthermore, since the task is open-domain and open-ended, there are many possible correct responses which may not match with a reference response~\cite{elikyilmaz2020EvaluationOT}. To tackle  these challenges, we propose an automatic metric for this task that does not use human references. The proposed metric \textbf{\metricname} is based on a classification model trained to classify a transition response as either \textit{positive}, that is, it is coherent to the context and smoothly transitions towards the target, or negative, that is, the response is either not coherent to the context or does not transition towards the target. 



% \begin{figure}[h]
%     \centering
%     \vspace{-.2pc}
%     \includegraphics[width=0.50\textwidth]{images/tc.png}
%     \vspace{-.5pc}
%     \caption{ We train a reference-less model-based metric \metricname{} to score the smoothness of a generate response wrt to dialogue context and target sentence. To train the metric, we synthesize hard negative examples using an enseble of techniques.}
%     \label{fig:tcsynth}
%     \vspace{-.2pc}
% \end{figure}


We use the gold transition response from the training dataset to create positive instances for training. For a positive instance with context $c$, target $t$ and response $r$, we create negative instances using the following mechanisms: 
%1) Sample a random response $r'$ from another instance, which makes it incoherent to the context $c$ and irrelevant to the target $t$. 2) Sample a random context $c'$, which makes $r$ incoherent to the $c'$, and 3) Sample a random target $t'$, which makes $r$ irrelevant to target $t'$. 
1) We hold two out of (c,t,r) constant while randomly sample the third one. For example, sample a random context $c'$, which makes $r$ incoherent to the $c'$,
% Since Otters training set is small, we use two more approaches to augment the negative instance set. In 4)
2) We use a GPT-2 model trained on Otters dataset to generate a response $r'$  coherent to $c$ but conditioned on a random target $t'$. %In 5) 
3) For a given target $t$, we chose a response $r'$ from the Otters training set which has $t$ as the target but context $c' \neq c$. 
We sample a maximum of 2 negative instance per mechanism and balance the count of positive and negative instances by  repeating positive instances. We fine-tune a pre-trained BERT-base~\cite{devlin-etal-2019-bert} model on these instances with binary cross entropy loss.
